Neural Compositional Rule Learning for Knowledge Graph Reasoning

Learning logical rules is critical to improving reasoning in KGs. This is due to their ability to provide logical and interpretable explanations when used for predictions, as well as their ability to generalize to other tasks, domains, and data. While recent methods have been proposed to learn logical rules, the majority of these methods are either restricted by their computational complexity and can not handle the large search space of large-scale KGs, or show poor generalization when exposed to data outside the training set. In this paper, we propose an end-to-end neural model for learning compositional logical rules called NCRL. NCRL detects the best compositional structure of a rule body, and breaks it into small compositions in order to infer the rule head. By recurrently merging compositions in the rule body with a recurrent attention unit, NCRL finally predicts a single rule head. Experimental results show that NCRL learns high-quality rules, as well as being generalizable. Specifically, we show that NCRL is scalable, efficient, and yields state-of-the-art results for knowledge graph completion on large-scale KGs. Moreover, we test NCRL for systematic generalization by learning to reason on small-scale observed graphs and evaluating on larger unseen ones.

==> contents/comparison_to_existing_works.tex <==
\section{Comparison with Existing Works}

\textbf{Neural Logic Programming Methods}:
There are also some recent methods based on neural logic programming such as Neural-LP~\cite{yang2017differentiable}, which are able to simultaneously learn logical rules and their weights in a differentiable way and RNNLogic~\cite{qu2020rnnlogic}, which is a principled probabilistic method, which separate rule generation and rule weight learning by introducing a rule generator and a reasoning predictor respectively. Both of the two different kinds of approaches are designed for KG completion task. However, these methods requires enumeration of all possible rules given a max rule length $T$. Therefore, it is hard for them to scale up to the exponentially large space of compositional rules, which severely limit their systematicity.

\textbf{Systematic Generalizable Methods}:
All the above methods cannot learn over smaller graphs where the rule paths are short and generalize to large-scale KG where the rule paths are long. 
% The capability to generalize to large-scale KG is called systematic generalization.
To overcome the problems of systematicity, Conditional Theorem Provers (CTPs) is proposed to learns an optimal rule selection strategy via gradient-based optimisation. For each sub-goal, a select module produces a smaller set of rules, which is then used during the proving mechanism. However, since the length of the learned rules influences the number of parameters of the model, it limits the capability of CTPs to handle the complicated rules whose depth is large. Another reinforcement learning based method - R5~\cite{lu2022r} is proposed to provide recurrent relational reasoning solution to learn compositional rules. However, R5 cannot generalize to KG completion task due to the lack of scalability. It requires pre-sampling for the paths that entails the query and it is time consuming to train even one paths with reinforcement learning framework. Considering that all the triples in a KG share the same training graph, even a relatively small scale KG contains a huge number of paths. In addition, R5 makes employ a hard decision mechanism for merging a relation pair into a single relation, which makes it challenging to handle the widely existing uncertainty in KGs. For example, given the rule body \emph{$\text{hasAunt}(x,z) \wedge \text{hasSister}(z, y)$}, both \emph{$\text{hasMother}(x, y)$} and \emph{$\text{hasAunt}(x, y)$} can be derived as the rule head. The inaccurate merging of a relation pair may result in the error propagation when generalize to longer paths.

==> contents/scoring_function.tex <==
\section{Similarity Measurement with Transformer}\label{sec:similarity measurement}
\textbf{Vanilla Transformer}
The traditional attention mechanism is a function:
\begin{equation}
Y = \text{Attn}(X,C) =\text{softmax}( \frac{XW_{Q}(CW_{K})^{T}}{\sqrt{d}})CW_{V}
\end{equation}
where the attention function $\text{Attn}(.): \mathbb{R}^{n \times d} \times \mathbb{R}^{m \times d} \rightarrow \mathbb{R}^{n \times d}$ takes two sequences as inputs: the query sequence $X \in  \mathbb{R}^{n \times d}$ with length $n$ and the context sequence $C \in \mathbb{R}^{m \times d}$ with length $m$, and output sequence $Y \in  \mathbb{R}^{n \times d}$ with the same length as the query sequence. $d$ is the embedding dimension, and $W_Q, W_K, W_V \in \mathbb{R}^{d \times d}$ are learnable parameters that project the input sequences into the space of query, key, and value: $Q = XW_Q, K = CW_K, V = CW_V$. Specifically, $ \text{softmax}(\frac{XW_{Q}(CW_{K})^{T}}{\sqrt{d}}) \in \mathbb{R}^{n \times m}$ is called the attention matrix which specifies the similarity scores between every pair of tokens in queries $X$ and contexts $C$. 

\textbf{Transformer for Rule Evaluation}
Note that the confidence of a logical rule can be measured based on the degree to which rule body and rule head are semantically consistent. Transformers provide a natural choice to measure the semantic relevance between two sequences of the inputs. By taking the representation of rule body as query and the representations of all predicates in KG as the key, Transformer is able to learn an attention $\mathbf{\theta}$ to estimate the similarity between rule body and each predicate in KG. In this case, the query sequence $X \in  \mathbb{R}^{1 \times d}$ contains only the embedding of rule body while the context sequence $C \in \mathbb{R}^{|R|+1 \times d}$ contains the embeddings of all predicates in KG. Note that we may not always find a proper target relation to represent a relation path. For example, given the relation path \emph{$[\text{hasBrother},\text{hasWife}]$}, we may not entail an existing relation to represent it. To accommodate unseen relations, we incorporate a ``null'' predicate into the context sequence, whose embedding is set as the embedding of rule body. $\mathbf{\theta}_{i}$ measures the degree to which the rule body semantically match with predicate $i$. The scaled dot-product attention computes the $\mathbf{\theta}$ as:

\begin{equation}
\begin{aligned}
\mathbf{\theta} = \text{softmax}( \frac{XW_{Q}(CW_{K})^{T}}{\sqrt{d}})
\end{aligned}
\end{equation}


Given the learned attention $\mathbf{\theta}$, we are able to compute a new representation of the rule body as a weighted combination of all predicates in KG each weighted by its attention weight.
\begin{equation}
\widehat{X} = \text{softmax}( \frac{XW_{Q}(CW_{K})^{T}}{\sqrt{d}})CW_{V}
\end{equation}
where $\widehat{X}$ is the new representation of the rule body and $\widehat{X} \in  \mathbb{R}^{1 \times d}$. We project the key and value to the same space by requiring $W_{V} = W_{K}$.


